Polaris: A G\"odel Agent Framework for Small Language Models through Experience-Abstracted Policy Repair

G\"odel agent realize recursive self-improvement: an agent inspects its own policy and traces and then modifies that policy in a tested loop. We introduce Polaris, G\"odel agent for compact models that performs policy repair via experience abstraction, turning failures into policy updates through a structured cycle of analysis, strategy formation, abstraction, and minimal code patch repair with conservative checks. Unlike response level self correction or parameter tuning, Polaris makes policy level changes with small, auditable patches that persist in the policy and are reused on unseen instances within each benchmark. As part of the loop, the agent engages in meta reasoning: it explains its errors, proposes concrete revisions to its own policy, and then updates the policy. To enable cumulative policy refinement, we introduce experience abstraction, which distills failures into compact, reusable strategies that transfer to unseen instances. On MGSM, DROP, GPQA, and LitBench (covering arithmetic reasoning, compositional inference, graduate-level problem solving, and creative writing evaluation), a 7-billion-parameter model equipped with Polaris achieves consistent gains over the base policy and competitive baselines.

==> figures/solver_update.tex <==
% \begin{figure*}[t]
% \centering
% % \resizebox{\linewidth}{!}{
% \includegraphics[width=\textwidth]{images/solver_functions.pdf}
% % }
% \caption{Example of how the policy is evolving across iterations. (Dataset: GPQA)}
% \label{fig: solver_figure}
% \end{figure*}


\includepdf[
  pages=1,            % adjust to your PDF
%   scale=0.95,           % fit as needed (or use fitpaper, width)
%   fitpaper=true,
  trim=0 100cm 0 0,
  pagecommand={}        % do NOT add anything on these pages
]{images/solver_functions.pdf}

% Import the last page and place the caption on it
% \includepdf[
%   pages=1,             % last page
%   scale=0.95,
%   pagecommand={
%     \captionsetup{type=figure}%
%     \captionof{figure}{A descriptive caption for the multi-page figure.}
%     \label{fig:my-multipage}
%   }
% ]{images/solver_functions.pdf}

==> tables/summary_exp3.tex <==

\begin{table}[!ht]
\small
\centering
\begin{tabular}{|l|r|r|r|}
\hline            & \multicolumn{1}{l|}{\textbf{MGSM}} & \multicolumn{1}{l|}{\textbf{DROP}} & \multicolumn{1}{l|}{\textbf{GPQA}} \\ \hline
\textbf{Successful}     & 5                                  & 3                                  & 4                                  \\ \hline
\textbf{No improvement} & 1                                  & 2                                  & 4                                  \\ \hline
\textbf{Unsuccessful}   & 4                                  & 5                                  & 2                                  \\ \hline
\textbf{Total}          & 10                                 & 10                                 & 10                                 \\ \hline
\end{tabular}
\caption{A summary of various runs of \textsc{Polaris} on datasets. For policy repair and experience abstraction, we consider a set of three failed instances from the validation set of each dataset ($N$=3).}
\label{tab: summary_exp3}
\end{table}





==> tables/summary_exp5.tex <==
\begin{table*}[!ht]
\centering
\begin{tabular}{|l|c|c|c|}
    \hline            & \textbf{MGSM} & \textbf{DROP} & \textbf{GPQA} \\ \hline
    \textbf{Successful}      & 4             & 3             & 5             \\ \hline
    \textbf{No improvement} & 1             & 1             & 2             \\ \hline
    \textbf{Unsuccessful}   & 5             & 6             & 3             \\ \hline
    \textbf{Total}          & 10             & 10             & 10             \\ \hline
\end{tabular}
\caption{A summary of various runs of \textsc{Polaris} on datasets. For policy repair and experience abstraction, we consider a set of five failed instances from the validation set of each dataset ($N$=5).}
\label{tab: summary_exp5}
\end{table*}

